The Skipped Beat: A Study of Sociopragmatic Understanding in LLMs for 64 Languages

Instruction tuned large language models (LLMs), such as ChatGPT, demonstrate remarkable performance in a wide range of tasks. Despite numerous recent studies that examine the performance of instruction-tuned LLMs on various NLP benchmarks, there remains a lack of comprehensive investigation into their ability to understand cross-lingual sociopragmatic meaning (SM), i.e., meaning embedded within social and interactive contexts. This deficiency arises partly from SM not being adequately represented in any of the existing benchmarks. To address this gap, we present SPARROW, an extensive multilingual benchmark specifically designed for SM understanding. SPARROW comprises 169 datasets covering 13 task types across six primary categories (e.g., anti-social language detection, emotion recognition). SPARROW datasets encompass 64 different languages originating from 12 language families representing 16 writing scripts. We evaluate the performance of various multilingual pretrained language models (e.g., mT5) and instruction-tuned LLMs (e.g., BLOOMZ, ChatGPT) on SPARROW through fine-tuning, zero-shot, and/or few-shot learning. Our comprehensive analysis reveals that existing open-source instruction tuned LLMs still struggle to understand SM across various languages, performing close to a random baseline in some cases. We also find that although ChatGPT outperforms many LLMs, it still falls behind task-specific finetuned models with a gap of 12.19 SPARROW score. Our benchmark is available at: https://github.com/UBC-NLP/SPARROW

==> append_related_work.tex <==
\section{Related Work}

\paragraph{Evaluation of LLMs.} 
Recently, instruction tuned LLMs (e.g., FLAN) have shown remarkable zero-shot performance on a wide range of NLP tasks and open-domain instruction-following tasks. ChatGPT, an LLM tuned with instructional data and RLHF by Open AI, has attracted more than $100$ million users since November 2022. There have been many attempts at holistic evaluation to better understand the capacities of ChatGPT and instruction tuned LLMs. \citet{qin-2023-chatgpt, systematic-2023-tahmid, zhong-2023-understand} utilize existing unified English evaluation benchmarks (such as GLUE, SuperGLUE, BigBench) to evaluate LLMs' capacities on various NLP tasks, including natural language inference, arithmetic and commonsense reasoning, question-answering, name-entity recognition, part-of-speech tagging, text summarization, etc. These studies find that although ChatGPT performs less effectively than the models finetuned specifically for each task, it demonstrates superior reasoning capabilities compared to other instruction tuned LLMs (e.g., FLAN). 
\citet{mega-2023-ahuja, bang2023multitask, systematic-2023-tahmid, beyond-2023-lai} evaluate LLMs on more diverse languages with existing multilingual evaluation benchmarks (such as XNLI, PAWS-X, XLSum) involving monolingual NLP tasks and crosslingual tasks (such as machine translation). Their findings indicate that there is still a large gap in performance of instruction tuned LLMs and ChatGPT, especially for low-resource languages and non-Latin languages. 
Moreover, we notice that SM is not adequately represented in these existing benchmarks and evaluations. As we summarize in Table~\ref{tab:related_compare}, these works only include a few SM tasks focusing on sentiment analysis. \citet{sentiment-2023-wang, sentiment-2023-zhang} investigate LLMs on more diverse SM tasks in English, such as aspect-based sentiment analysis and offensive language detection. \citet{das-2023-evaluating} evaluate the ability of ChatGPT in detecting hate speech across 11 languages. 
% \citet{qin-2023-chatgpt} evaluates ChatGPT on $20$ English NLP datasets encompassing seven task categories in a zero-shot setting. They find that ChatGPT demonstrates superior reasoning capabilities compared to other instructed tuned LLMs (e.g., FLAN) 
We find the closest work to our paper is the work by \citet{ziems-2023-can}, which investigates the zero-shot ability of ChatGPT across a broad spectrum of English computational social science (CSS) benchmarks encompassing various subject areas, such as sociology, psychology, and linguistics. However, they solely focus on English CSS tasks. Compare to previous works, our paper aims to investigate more diverse SM tasks with massively diverse languages and datasets. To achieve our goal, we construct an evaluation benchmark for SM (i.e., SPARROW). We now discuss how our proposed benchmark distinguishes it from existing work. 
%They find that ChatGPT demonstrates poor performance on tasks characterized by structural complexity (e.g., event arguments) or those that entail subjective expert taxonomies (e.g., hate, empathy).

% \citet{ziems-2023-can} investigate the zero-shot ability of ChatGPT across a broad spectrum of computational social science benchmarks encompassing various subject areas, including sociology, psychology, literature, history, linguistics, and political science. They find that ChatGPT demonstrates poor performance on tasks characterized by structural complexity (e.g., event arguments) or those that entail subjective expert taxonomies (e.g., hate, empathy). However, it attains high performance on tasks that involve either objective ground truth (like fact-checking tasks) or explicit definition labels (e.g., anger in emotion detection). Furthermore, it is observed that ChatGPT exhibits a tendency to predict a neutral label that is easily recognized in colloquial language (e.g., stereotype in the hate speech detection task), instead of utilizing a more precise label derived from the provided taxonomy (e.g., white grievance). \citet{qin-2023-chatgpt} evaluates Chat-GPT on 20 NLP datasets encompassing seven task categories in a zero-shot setting. Although Chat-GPT performs less effectively than models fine-tuned specifically for each task, it demonstrates superior reasoning capabilities compared to other instructed fine-tuned models (e.g., FLAN) in natural language inference, arithmetic reasoning, and question-answering tasks.
% \citet{gilardi2023chatgpt} use a dataset of 2,382 tweets to show that in some cases, the performance of ChatGPT is better than crow-workers. They implemented 5 different classification tasks, including, relevance, topic detection, stance detection, general frame detection, and policy frame detection. The evaluation of the outcomes is based on both accuracy and intercoder agreement. The findings reveal that ChatGPT achieves superior accuracy in four out of the five tasks and outperforms human workers in all tasks when it comes to intercoder agreement.
% \citet{bang2023multitask} present a framework that offers a quantitative evaluation of interactive language models (LLMs). They assess the performance of ChatGPT using 23 datasets that encompass a wide range of tasks in multitask, multilingual, and multimodal settings. The findings indicate that ChatGPT surpasses zero-shot learning LLMs on the majority of tasks and even outperforms fine-tuned models on certain tasks. However, ChatGPT is prone to hallucination issues, generating more extrinsic hallucinations compared to other LLMs.
% \citet{lai2023chatgpt} perform an assessment of ChatGPT across seven distinct tasks, including part-of-speech tagging, named entity recognition, relation extraction, natural language inference, question answering, commonsense reasoning, and summarization. The evaluation encompasses a wide range of languages, incorporating 37 diverse linguistic backgrounds with varying levels of resources available (high, medium, low, and extremely low). The findings indicate that ChatGPT's performance in a multilingual setting is significantly poor. 

\input{table_fig/related_work}

\paragraph{Evaluation Benchmarks for SM.}
To facilitate the model comparison, many previous works have introduced unified benchmarks, such as GLUE~\cite{wang-etal-2018-glue}, SentEval~\cite{conneau-2018-senteval}, XTREME~\cite{hu-2020-xtreme}, and XGLUE~\cite{liang-2020-xglue}. These benchmarks include a wide range of NLP tasks (e.g., natural language inference, text semantic similarity, question generation) but use only sentiment analysis as a representation of SM tasks. Recent studies have started to construct unified benchmarks focusing on evaluating SM with social media data. \citet{barbieri-2020-tweeteval} introduce TweetEval benchmark that contains seven English datasets of six SM tasks. \citet{sentieval-2023-zhang} develop SentiEval benchmark that involves $26$ English datasets of $13$ sentiment-related tasks (e.g., sentence-level sentiment analysis, irony detection). Beyond English, NusaX~\cite{nusax-2020-genta}, NaijaSenti~\cite{muhammad-2022-naijasenti}, and AfriSenti~\cite{afrisenti-2023-muhammad} propose a new benchmark for sentiment analysis with eight Indonesian languages, four African languages, and $14$ African languages respectively. UMSAB introduced by \citet{barbieri-etal-2022-xlm} contains $11$ sentiment analysis datasets in $11$ languages. For detecting anti-social online comments, \citet{risch-etal-2021-toxic} introduces a unified toxic comment collection that contains $43$ datasets of six anti-social detection tasks in $14$ languages. Compare to previous work, our SPARROW benchmark includes more diverse SM tasks and languages from more diverse social media platforms, as Figure~\ref{fig:sparrow_compare} shows.  


==> table_fig/antisocial_prompt.tex <==
% \begin{table*}[h]
% \centering 
% \tiny
% \begin{tabular}{p{0.1\linewidth}l}
%  \toprule
% \textbf{Dataset}	 & \textbf{Prompt} \\ \midrule
% Dang-ara\textsubscript{Als} 	 & \makecell[l]{\{Content\} \\ Question: Is the language of this sentence \{labels\}? \\ Answer: } \\ \midrule
% Aggr-hin\textsubscript{Kum} 	 & \multirow{24}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\
% Hate-eng\textsubscript{Dav} 	 & \\
% Hate-eng\textsubscript{Was} 	 & \\ 
% Hate-ara\textsubscript{Ala} 	 & \\ 
% Hate-ita\textsubscript{Bos}\textsuperscript{$\star$} 	 & \\ 
% Hate-fil\textsubscript{Cab} 	 & \\ 
% Hate-ara\textsubscript{Mul} 	 & \\ 
% Hate-eng\textsubscript{Bas} 	 & \\ 
% Hate-spa\textsubscript{Bas} 	 & \\ 
% Hate-por\textsubscript{For} 	 & \\ 
% Hate-pol\textsubscript{Pta} 	 & \\ 
% Hate-kor\textsubscript{Moo} 	 & \\ 
% Hate-ara\textsubscript{Mub} 	 & \\ 
% Hate-zho\textsubscript{Den} 	 & \\ 
% Hate-kor\textsubscript{Jeo} 	 & \\ 
% Hate-tel\textsubscript{Mar} 	 & \\ 
% Sexi-fre\textsubscript{Chi} 	 & \\
% Offe-eng\textsubscript{Zam} 	 & \\ 
% Offe-ara\textsubscript{Zam} 	 & \\ 
% Offe-dan\textsubscript{Zam} 	 & \\ 
% Offe-ell\textsubscript{Zam} 	 & \\ 
% Offe-tur\textsubscript{Zam} 	 & \\ 
% Offe-ara\textsubscript{Mub} 	 & \\ 
% Offe-slv\textsubscript{Nov} 	 & \\ \midrule
% Offe-T-kan\textsubscript{Cha} 	 & \multirow{3}{*}{\makecell[l]{\{Content\} \\ Question: Does this offensive text target \{labels\}? \\ Answers: }} \\
% Offe-G-eng\textsubscript{Zam} 	 & \\ 
% Hate-T-kor\textsubscript{Jeo} 	 & \\ \midrule
% Hate-G-ara\textsubscript{Ous} 	 & \multirow{3}{*}{\makecell[l]{\{Content\} \\ Question: Does this hate speech target \{labels\}? \\ Answer: }} \\
% Hate-G-fre\textsubscript{Ous} 	 & \\
%  & \\ \midrule
% Offe-T-eng\textsubscript{Zam} 	 & \makecell[l]{\{Content\} \\ Question: Is this offensive text \{labels\} insult? \\ Answer: } \\ \midrule
% Hate-T-ara\textsubscript{Ous} 	 & \multirow{3}{*}{\makecell[l]{\{Content\} \\ Question: Does this hate speech text insult against people based on their attribute of \{labels\}? \\ Answer: }} \\
% Hate-T-fre\textsubscript{Ous} 	 & \\ 
%  & \\ \midrule
% Hate-T-ben\textsubscript{Kar} 	 & \makecell[l]{\{Content\} \\ Question: Does this text express \{labels\}? \\ Answer: } \\ \midrule
% Offe-T-mal\textsubscript{Cha} 	 & \multirow{3}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence hate speech or not? If yes, does this sentence target individual, group or not? \\ Answer: }} \\
% Offe-T-tam\textsubscript{Cha} 	 & \\
%  & \\
% \bottomrule 
% \end{tabular}
% \caption{Irony.}\label{tab:irony_prompt}
% \end{table*}

\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{ll}
 \toprule
\textbf{Dataset}	 & \textbf{Prompt} \\ \midrule
Dang-ara\textsubscript{Als} 	 & \makecell[l]{\{Content\} \\ Question: Is the language of this sentence \{labels\}? \\ Answer: } \\ \midrule
Aggr-hin\textsubscript{Kum}, Hate-eng\textsubscript{Dav}, Hate-eng\textsubscript{Was}, Hate-ara\textsubscript{Ala}, Hate-ita\textsubscript{Bos}\textsuperscript{$\star$}, Hate-fil\textsubscript{Cab} 	 & \multirow{4}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\
Hate-ara\textsubscript{Mul}, Hate-eng\textsubscript{Bas}, Hate-spa\textsubscript{Bas}, Hate-por\textsubscript{For}, Hate-pol\textsubscript{Pta}, Hate-kor\textsubscript{Moo} 	 & \\
Hate-ara\textsubscript{Mub}, Hate-zho\textsubscript{Den}, Hate-kor\textsubscript{Jeo}, Hate-tel\textsubscript{Mar}, Sexi-fre\textsubscript{Chi}, Offe-eng\textsubscript{Zam} 	 & \\ 
Offe-ara\textsubscript{Zam}, Offe-dan\textsubscript{Zam}, Offe-ell\textsubscript{Zam}, Offe-tur\textsubscript{Zam}, Offe-ara\textsubscript{Mub}, Offe-slv\textsubscript{Nov} 	 & \\ \midrule
Offe-T-kan\textsubscript{Cha}, Offe-G-eng\textsubscript{Zam}, Hate-T-kor\textsubscript{Jeo} 	 & \makecell[l]{\{Content\} \\ Question: Does this offensive text target \{labels\}? \\ Answers: } \\ \midrule
Hate-G-ara\textsubscript{Ous}, Hate-G-fre\textsubscript{Ous} 	 & \makecell[l]{\{Content\} \\ Question: Does this hate speech target \{labels\}? \\ Answer: } \\ \midrule
Offe-T-eng\textsubscript{Zam} 	 & \makecell[l]{\{Content\} \\ Question: Is this offensive text \{labels\} insult? \\ Answer: } \\ \midrule
Hate-T-ara\textsubscript{Ous}, Hate-T-fre\textsubscript{Ous} 	 & \makecell[l]{\{Content\} \\ Question: Does this hate speech text insult against people based on their attribute of \{labels\}? \\ Answer: } \\ \midrule
Hate-T-ben\textsubscript{Kar} 	 & \makecell[l]{\{Content\} \\ Question: Does this text express \{labels\}? \\ Answer: } \\ \midrule
Offe-T-mal\textsubscript{Cha}, Offe-T-tam\textsubscript{Cha} 	 & \makecell[l]{\{Content\} \\ Question: Is this sentence hate speech or not? If yes, does this sentence target individual, group or not? \\ Answer: } \\
\bottomrule 
\end{tabular}
\caption{Antisocial.}\label{tab:antisocial_prompt}
\end{table*}



==> table_fig/datasum.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[h]
\tiny
\begin{tabular}{@{}llllllp{0.2\linewidth}llll@{}}
\toprule
dataset                           & citation                                                  & language & Source / domain           & Year & \# label & labels                                                                                                                                                                                                                                                                           & train  & dev   & test  & Publicly accessable? \\ \midrule
accident-2020-hamoui-ar           & \cite{hamoui-etal-2020-flodusta}         & ar       & Tweets                    & 2020 & 4        & {Immediate\_Accident, Immediate\_Dust\_Storm, Immediate\_Flood, Irrelevant\_None-event}                                                                                                                                                                                        & 4284   & 536   & 536   & Yes                  \\
agressive-2018-kumar-hi           & \cite{kumar-2018-aggression}             & hi       & Twitter and Facebook      & 2018 & 2        & {Aggressive, Not}                                                                                                                                                                                                                                                              & 9306   & 1163  & 1164  & Yes                  \\
crisislext6-2014-olteanu-en       & \cite{olteanu2014crisislex}              & en       & Twitter                   & 2014 & 2        & {Not, Related}                                                                                                                                                                                                                                                                 & 48065  & 6008  & 6009  & Yes                  \\
dangerous-2020-alshehri-ar        & \cite{alshehri-etal-2020-understanding}  & ar       & Twitter                   & 2020 & 2        & {Dangerous, Not}                                                                                                                                                                                                                                                               & 3474   & 615   & 663   & Yes                  \\
emotion-1994-scherer-en           & \cite{wallbott1986universal}             & en       & Questionnaire             & 1986 & 7        & {Anger, Disgust, Fear, Guilt, Joy, Sadness, Shame}                                                                                                                                                                                                                             & 6132   & 767   & 767   & Yes                  \\
emotion-2018-cynar-fi             & \cite{kajava2018cross}                   & fi       & Subtitle                  & 2016 & 8        & {Anger, Anticipation, Disgust, Fear, Joy, Sadness, Surprise, Trust}                                                                                                                                                                                                            & 5197   & 577   & 653   & Yes                  \\
emotion-2018-cynar-fr             & \cite{kajava2018cross}                   & fr       & Subtitle                  & 2016 & 8        & {Anger, Anticipation, Disgust, Fear, Joy, Sadness, Surprise, Trust}                                                                                                                                                                                                            & 5198   & 577   & 653   & Yes                  \\
emotion-2018-cynar-it             & \cite{kajava2018cross}                   & it       & Subtitle                  & 2016 & 8        & {Anger, Anticipation, Disgust, Fear, Joy, Sadness, Surprise, Trust}                                                                                                                                                                                                            & 5197   & 577   & 653   & Yes                  \\
emotion-2018-mohammad-en          & \cite{mohammad-2018-semeval}             & en       & Twitter                   & 2018 & 4        & {Anger, Joy, Optimism, Sadness}                                                                                                                                                                                                                                                & 3257   & 374   & 1421  & Yes                  \\
emotion-2018-semeval-es           & \cite{mohammad-2018-semeval}             & es       & Twitter                   & 2018 & 4        & {Anger, Fear, Joy, Sadness}                                                                                                                                                                                                                                                    & 4541   & 793   & 2616  & Yes                  \\
emotion-2020-abdul-ar             & \cite{mageed-2020-aranet}               & ar       & Twitter                   & 2016 & 8        & {Anger, Anticipation, Disgust, Fear, Joy, Sadness, Surprise, Trust}                                                                                                                                                                                                            & 50000  & 910   & 941   & Yes                  \\
emotion-2020-nguyen-vi            & \cite{ho2019emotion}                     & vi       & Facebook                  & 2019 & 7        & {Anger, Disgust, Fear, Joy, Others, Sadness, Surprise}                                                                                                                                                                                                                         & 5548   & 686   & 693   & Yes                  \\
emotion-2020-plaza-en             & \cite{plaza-del-arco-etal-2020-emoevent} & en       & Twitter                   & 2020 & 7        & {Anger, Disgust, Fear, Joy, Others, Sadness, Surprise}                                                                                                                                                                                                                         & 5842   & 730   & 731   & Yes                  \\
emotion-2020-plaza-es             & \cite{plaza-del-arco-etal-2020-emoevent} & es       & Twitter                   & 2020 & 7        & {Anger, Disgust, Fear, Joy, Others, Sadness, Surprise}                                                                                                                                                                                                                         & 6727   & 841   & 841   &                      \\
emotion-2020-wilie-in             & \cite{wong-2020-indonlu}                 & in       & Twitter                   & 2018 & 5        & {Anger, Fear, Happy, Love, Sadness}                                                                                                                                                                                                                                            & 3169   & 352   & 440   & Yes                  \\
emotion-2021-feelit-it            & \cite{bianchi2021feel}                  & it       & Twitter                   & 2021 & 4        & {Anger, Fear, Joy, Sadness}                                                                                                                                                                                                                                                    & 1629   & 204   & 204   & Yes                  \\
emotion-2021-ohman-fi             & \cite{ohman2020xed}                      & fi       & Subtitle                  & 2020 & 8        & {Anger, Anticipation, Disgust, Fear, Joy, Sadness, Surprise, Trust}                                                                                                                                                                                                            & 8864   & 1118  & 1086  & Yes                  \\
goemotion-2020-demszky-en         & \cite{demszky2020goemotion}              & en       & Reddit                    & 2020 & 27       & {Admiration, Amusement, Anger, Annoyance, Approval, Caring, Confusion, Curiosity, Desire, Disappointment, Disapproval, Disgust, Embarrassment, Excitement, Fear, Gratitude, Grief, Joy, Love, Nervousness, Optimism, Pride, Realization, Relief, Remorse, Sadness5, Surprise6} & 23485  & 2956  & 2984  & Yes                  \\
hate-2016-waseem-en               & \cite{waseem-2016-hateful}               & en       & Twitter                   & 2016 & 3        & {Not, Racism, Sexism}                                                                                                                                                                                                                                                          & 8683   & 1086  & 1085  & Yes                  \\
hate-2017-david-en                & \cite{davidson-2017-hateoffensive}       & en       & Twitter                   & 2017 & 3        & {Hate, Not, Offensive}                                                                                                                                                                                                                                                         & 19826  & 2478  & 2479  & Yes                  \\
hate-2018-azalden-ar              & \cite{alakrot2018dataset}                & ar       & YouTube comment           & 2017 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 9014   & 1127  & 1127  & Yes                  \\
hate-2018-evalita-it              & \cite{bosco2018overview}                 & it       & Twitter                   & 2018 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 2700   & 300   & 1000  & Yes                  \\
hate-2019-mulki-ar                & \cite{mulki2019hsab}                     & ar       & Twitter                   & 2019 & 3        & {Abusive, Hate, Not}                                                                                                                                                                                                                                                           & 4208   & 468   & 1170  & Yes                  \\
hate-2019-ptaszynski-pl           & \cite{ptaszynski2019results}             & pl       & Twitter                   & 2019 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 9037   & 1004  & 1000  & Yes                  \\
hate-2020-cruz-fil                & \cite{cabasag2019hate}                   & fil      & Twitter                   & 2016 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 10000  & 4232  & 4232  & Yes                  \\
hate-2020-karim-bn                & \cite{karim2020deephateexplainer}        & bn       & Multiple online platforms & 2020 & 4        & {Geopolitical, Personal, Political, Religion}                                                                                                                                                                                                                                  & 4558   & 570   & 570   & Yes                  \\
hate-2020-moon-ko                 & \cite{moon-etal-2020-beep}               & ko       & News comments             & 2020 & 3        & {Hate, Not, Offensive}                                                                                                                                                                                                                                                         & 7106   & 790   & 471   & Yes                  \\
hate-2020-mubarak-ar              & \cite{mubarak-etal-2020-overview}        & ar       & Twitter                   & 2020 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 6839   & 1000  & 2000  & Yes                  \\
hate-2022-deng-zh                 & \cite{deng-2022-cold}                    & zh       & Weibo                     & 2022 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 25726  & 6431  & 5323  & Yes                  \\
hate-2022-jeong-ko                & \cite{jeong-2022-kold}                   & ko       & News and YouTube comments & 2022 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 32343  & 4043  & 4043  & Yes                  \\
hate-2023-marreddy-te             & \cite{mounika-2022-resource}             & te       & Multiple online platforms & 2022 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 24599  & 3510  & 7033  & Yes                  \\
hate-group-2019-ousidhoum-ar      & \cite{ousidhoum2019multilingual}         & ar       & Twitter                   & 2019 & 13       & {African\_descent, Arabs, Asians, Christian, Gay, Immigrants, Indian/hindu, Individual, Jews, Muslims, Others, Refugees, Women}                                                                                                                                                & 2682   & 334   & 335   & Yes                  \\
hate-group-2019-ousidhoum-fr      & \cite{ousidhoum2019multilingual}         & fr       & Twitter                   & 2019 & 16       & {African\_descent, Arabs, Asians, Christian, Gay, Gispanics, Immigrants, Indian/hindu, Individual, Jews, Left\_wing\_people, Muslims, Others, Refugees, Special\_needs, Women}                                                                                                 & 3211   & 401   & 402   & Yes                  \\
hate-target-2019-ousidhoum-ar     & \cite{ousidhoum2019multilingual}         & ar       & Twitter                   & 2019 & 4        & {Gender, Origin, Others, Religion}                                                                                                                                                                                                                                             & 2682   & 334   & 336   & Yes                  \\
hate-target-2019-ousidhoum-fr     & \cite{ousidhoum2019multilingual}         & fr       & Twitter                   & 2019 & 6        & {Disability, Gender, Origin, Others, Religion, Sexual\_Orientation}                                                                                                                                                                                                            & 3211   & 401   & 402   & Yes                  \\
hate-target-2022-jeong-ko         & \cite{jeong-2022-kold}                   & ko       & News and YouTube comments & 2022 & 4        & {Group, Individual, Other, Untargeted}                                                                                                                                                                                                                                         & 16239  & 2049  & 2022  & Yes                  \\
hateval-2019-basile-en            & \cite{basile-2019-semeval}               & en       & Twitter                   & 2019 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 9000   & 1000  & 3000  & Yes                  \\
hateval-2019-basile-es            & \cite{basile-2019-semeval}               & es       & Twitter                   & 2019 & 2        & {Hate, Not}                                                                                                                                                                                                                                                                    & 4500   & 500   & 1600  & Yes                  \\
humor-2018-khandelwal-hi          & \cite{aggarwal2020sarcasm}               & hi       & Twitter                   & 2018 & 2        & {Humor, Not}                                                                                                                                                                                                                                                                   & 4187   & 524   & 523   & Yes                  \\
humor-2019-blinov-ru              & \cite{blinov-2019-large}                 & ru       & Multiple online platforms & 2018 & 2        & {Humor, Not}                                                                                                                                                                                                                                                                   & 251416 & 61794 & 1877  & Yes                  \\
humor-2021-chiruzzo-es            & \cite{chiruzzo2021overview}              & es       & Twitter                   & 2019 & 2        & {Humor, Not}                                                                                                                                                                                                                                                                   & 24000  & 6000  & 6000  & Yes                  \\
humor-2021-meaney-en              & \cite{meaney2021hahackathon}             & en       & Twitter                   & 2021 & 2        & {Humor, Not}                                                                                                                                                                                                                                                                   & 8000   & 1000  & 1000  & Yes                  \\
irony-2014-barbieri-it            & \cite{barbieri2014italian}               & it       & Twitter                   & 2013 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 19736  & 2467  & 2467  & Yes                  \\
irony-2016-barbieri-es            & \cite{barbieri2016overview}              & es       & Twitter                   & 2014 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 6669   & 741   & 1997  & Yes                  \\
irony-2018-hee-en                 & \cite{van-hee2018semeval}                & en       & Twitter                   & 2018 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 3450   & 384   & 784   & Yes                  \\
irony-2018-ironita-it             & \cite{cignarella2018overview}           & it       & Twitter                   & 2018 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 3579   & 398   & 872   & Yes                  \\
irony-2018-vijay-hi               & \cite{vijay-2018-dataset-irony}          & hi       & Twitter                   & 2018 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 2217   & 277   & 277   & Yes                  \\
irony-2019-ghanem-ar              & \cite{idat2019ghanem}                    & ar       & Twitter                   & 2019 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 3622   & 402   & 1006  & Yes                  \\
irony-2019-irosva-es              & \cite{ortega2019overview}               & es       & Twitter                   & 2019 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 2160   & 240   & 600   & Yes                  \\
irony-2020-golazizian-fa          & \cite{golazizian2020mirasirony}          & fa       & Twitter                   & 2019 & 2        & {Irony, Not}                                                                                                                                                                                                                                                                   & 2352   & 295   & 294   & No                   \\
irony-2020-xiang-zh               & \cite{xiang2020ciron}                    & zh       & Weibo                     & 2020 & 5        & {Insufficient\_Evidence, Irony, Not, Unlikely\_Ironic, Weakly\_Irony}                                                                                                                                                                                                          & 7014   & 876   & 876   & Yes                  \\
irony-type-2018-hee-en            & \cite{van-hee2018semeval}                & en       & Twitter                   & 2018 & 4        & {Ironic\_by\_clash, Not, Other\_irony, Situational\_irony}                                                                                                                                                                                                                     & 3450   & 384   & 784   & Yes                  \\
offense-2022-chakravarthi-kn      & \cite{chakravarthi-2022-dravidian}       & kn       & YouTube comment           & 2019 & 5        & {Group, Individual, Not, Others, Untargeted}                                                                                                                                                                                                                                   & 4694   & 586   & 593   & Yes                  \\
offense-2022-chakravarthi-ml      & \cite{chakravarthi-2022-dravidian}       & ml       & YouTube comment           & 2019 & 4        & {Group, Individual, Not, Untargeted}                                                                                                                                                                                                                                           & 14723  & 1836  & 1844  & Yes                  \\
offense-2022-chakravarthi-ta      & \cite{chakravarthi-2022-dravidian}       & ta       & YouTube comment           & 2019 & 5        & {Group, Individual, Not, Others, Untargeted}                                                                                                                                                                                                                                   & 33685  & 4216  & 4232  & Yes                  \\
offensive-2019-zampieri-en        & \cite{zampieri-2019-predicting}          & en       & Twitter                   & 2019 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 11916  & 1324  & 860   & Yes                  \\
offensive-2020-mubarak-ar         & \cite{mubarak2020overview}               & ar       & Twitter                   & 2020 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 6839   & 1000  & 2000  & Yes                  \\
offensive-2020-zampieri-ar        & \cite{zampieri-etal-2020-semeval}        & ar       & Twitter                   & 2019 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 7055   & 784   & 1827  & Yes                  \\
offensive-2020-zampieri-da        & \cite{zampieri-etal-2020-semeval}        & da       & Multiple online platforms & 2019 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 2664   & 296   & 329   & Yes                  \\
offensive-2020-zampieri-el        & \cite{zampieri-etal-2020-semeval}        & el       & Twitter                   & 2019 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 7869   & 874   & 1544  & Yes                  \\
offensive-2020-zampieri-tr        & \cite{zampieri-etal-2020-semeval}        & tr       & Twitter                   & 2019 & 2        & {Not, Offensive}                                                                                                                                                                                                                                                               & 28149  & 3128  & 3515  & Yes                  \\
offensive-2021--sl                & \cite{kralj2021slovenian}                & sl       & Twitter                   & 2020 & 4        & {Appropriate, Inappropriate, Not, Offensive}                                                                                                                                                                                                                                   & 65021  & 8127  & 8128  & Yes                  \\
offensive-group-2019-zampieri-en  & \cite{zampieri-2019-predicting}          & en       & Twitter                   & 2019 & 3        & {Group, Individual, Others}                                                                                                                                                                                                                                                    & 3485   & 391   & 213   & Yes                  \\
offensive-target-2019-zampieri-en & \cite{zampieri-2019-predicting}          & en       & Twitter                   & 2019 & 2        & {Targeted, Untargeted}                                                                                                                                                                                                                                                         & 3963   & 437   & 240   & Yes                  \\
sarcasm-2012-walker-en            & \cite{walker2012corpus}                  & en       & Debate Forums             & 2012 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 900    & 100   & 995   & Yes                  \\
sarcasm-2013-riloff-en            & \cite{riloff2013sarcasm}                 & en       & Twitter                   & 2013 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 1413   & 177   & 177   & Yes                  \\
sarcasm-2014-ptacek-cs            & \cite{ptavcek2014sarcasm}                & cs       & Twitter                   & 2013 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 3977   & 497   & 497   & Yes                  \\
sarcasm-2014-ptacek-en            & \cite{ptavcek2014sarcasm}                & en       & Twitter                   & 2013 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 71433  & 8929  & 8930  & Yes                  \\
sarcasm-2015-bamman-en            & \cite{bamman2015contextualized}          & en       & Twitter                   & 2015 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 11864  & 1483  & 1484  & Yes                  \\
sarcasm-2015-rajadesingan-en      & \cite{rajadesingan2015sarcasm}           & en       & Twitter                   & 2015 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 41261  & 5158  & 5158  & Yes                  \\
sarcasm-2016-oraby-en             & \cite{oraby2016creating}                 & en       & Debate Forums             & 2016 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 900    & 100   & 2260  & Yes                  \\
sarcasm-2018-araujodasilva-pt     & \cite{fabio-2018-irony}                  & pt       & Twitter                   & 2018 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 11783  & 1473  & 1473  & Yes                  \\
sarcasm-2020-aggarwal-hi          & \cite{aggarwal2020sarcasm}               & hi       & Twitter                   & 2020 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 73719  & 9215  & 9215  & Yes                  \\
sarcasm-2020-farha-ar             & \cite{abu-farha-magdy-2020-arabic}       & ar       & Twitter                   & 2020 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 7593   & 844   & 2110  & Yes                  \\
sarcasm-2021-abufarha-ar          & \cite{abufarha-etal-2021-arsarcasm-v2}   & ar       & Twitter                   & 2020 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 11293  & 1255  & 3000  & Yes                  \\
sarcasm-2022-wen-zh               & \cite{gong-2020-design}                  & zh       & News comments             & 2019 & 2        & {Not, Sarcasm}                                                                                                                                                                                                                                                                 & 3978   & 497   & 497   & No                   \\
sentiment-2005-pang-en            & \cite{pang2005seeing}                    & en       & Moview review             & 2005 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 8529   & 1066  & 1067  & Yes                  \\
sentiment-2008-tan-zh             & \cite{tan-2008-empirical}                & zh       & Multiple online platforms & 2008 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 9600   & 1200  & 1200  & Yes                  \\
sentiment-2013-kosac-ko           & \cite{jang-2013-kosac}                   & ko       & News articles             & 2013 & 4        & {Complex, Negative, Neutral, Positive}                                                                                                                                                                                                                                         & 4187   & 523   & 524   & No                   \\
sentiment-2013-socher-en          & \cite{socher-2013-recursive}             & en       & Moview review             & 2013 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 6920   & 872   & 1821  & Yes                  \\
sentiment-2015-patra-bn           & \cite{patra-2018-sentiment}              & bn       & Twitter                   & 2015 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 2250   & 250   & 3038  & No                   \\
sentiment-2015-patra-hi           & \cite{patra-2018-sentiment}              & hi       & Twitter                   & 2015 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 11642  & 1293  & 5525  & No                   \\
sentiment-2016-igor-bg            & \cite{mozetivc2016multilingual}          & bg       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 22184  & 2773  & 2773  & Yes                  \\
sentiment-2016-igor-bs            & \cite{mozetivc2016multilingual}          & bs       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 16335  & 2042  & 2042  & Yes                  \\
sentiment-2016-igor-de            & \cite{mozetivc2016multilingual}          & de       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 42010  & 5251  & 5252  & Yes                  \\
sentiment-2016-igor-en            & \cite{mozetivc2016multilingual}          & en       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 34538  & 4317  & 4318  & Yes                  \\
sentiment-2016-igor-es            & \cite{mozetivc2016multilingual}          & es       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 122410 & 15301 & 15302 & Yes                  \\
sentiment-2016-igor-hr            & \cite{mozetivc2016multilingual}          & hr       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 52971  & 6621  & 6622  & Yes                  \\
sentiment-2016-igor-hu            & \cite{mozetivc2016multilingual}          & hu       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 32717  & 4089  & 4090  & Yes                  \\
sentiment-2016-igor-pl            & \cite{mozetivc2016multilingual}          & pl       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 87941  & 10993 & 10992 & Yes                  \\
sentiment-2016-igor-pt            & \cite{mozetivc2016multilingual}          & pt       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 39525  & 4941  & 4940  & Yes                  \\
sentiment-2016-igor-ru            & \cite{mozetivc2016multilingual}          & ru       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 32941  & 4117  & 4118  & Yes                  \\
sentiment-2016-igor-sk            & \cite{mozetivc2016multilingual}          & sk       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 30694  & 3837  & 3837  & Yes                  \\
sentiment-2016-igor-sl            & \cite{mozetivc2016multilingual}          & sl       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 59924  & 7491  & 7490  & Yes                  \\
sentiment-2016-igor-sq            & \cite{mozetivc2016multilingual}          & sq       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 29375  & 3672  & 3672  & Yes                  \\
sentiment-2016-igor-sr            & \cite{mozetivc2016multilingual}          & sr       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 22124  & 2765  & 2766  & Yes                  \\
sentiment-2016-igor-sv            & \cite{mozetivc2016multilingual}          & sv       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 27277  & 3409  & 3410  & Yes                  \\
sentiment-2016-rei-de             & \cite{rei2016multilingual}               & de       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 2701   & 337   & 338   & Yes                  \\
sentiment-2016-rei-es             & \cite{rei2016multilingual}               & es       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 6099   & 763   & 762   & Yes                  \\
sentiment-2016-rei-it             & \cite{rei2016multilingual}               & it       & Twitter                   & 2016 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 6818   & 853   & 852   & Yes                  \\
sentiment-2017-rosenthal-en       & \cite{rosenthal-2017-semeval}            & en       & Twitter                   & 2017 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 42756  & 4751  & 12284 & Yes                  \\
sentiment-2018-amram-he           & \cite{amram-etal-2018-representations}   & he       & Facebook                  & 2018 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 8951   & 995   & 2488  & Yes                  \\
sentiment-2018-brum-pt            & \cite{brum-2018-building}                & pt       & Twitter                   & 2017 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 45127  & 5585  & 5637  & Yes                  \\
sentiment-2018-cynar-fi           & \cite{kajava2018cross}                   & fi       & Subtitle                  & 2016 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 5197   & 577   & 653   & Yes                  \\
sentiment-2018-cynar-fr           & \cite{kajava2018cross}                   & fr       & Subtitle                  & 2016 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 5198   & 577   & 653   & Yes                  \\
sentiment-2018-cynar-it           & \cite{kajava2018cross}                   & it       & Subtitle                  & 2016 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 5197   & 577   & 653   & Yes                  \\
sentiment-2018-velldal-no         & \cite{velldal-etal-2018-norec}           & no       & Online reviews            & 2018 & 6        & {Negative1, Negative2, Negative3, Positive4, Positive5, Positive6}                                                                                                                                                                                                             & 34903  & 4360  & 4351  & Yes                  \\
sentiment-2019-koco-pl            & \cite{kocon-etal-2019-multi}             & pl       & Customer reviews          & 2019 & 4        & {Complex, Negative, Neutral, Positive}                                                                                                                                                                                                                                         & 5170   & 574   & 1217  & Yes                  \\
sentiment-2019-suriyawongkul-th   & \cite{suriyawongkul-2019-pythainlp}      & th       & Facebook                  & 2019 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 21152  & 2362  & 2614  & Yes                  \\
sentiment-2019-weibo-zh           & \cite{wan-2020-s2ap}                     & zh       & Weibo                     & 2019 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 95990  & 11999 & 11999 & Yes                  \\
sentiment-2020-ashrafi-fa         & \cite{ashrafi2020mirasopinion}           & fa       & Online comments           & 2020 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 75094  & 9387  & 9387  & No                   \\
sentiment-2020-oyewusi-pcm        & \cite{oyewusi-2020-semantic}             & pcm      & Twitter                   & 2020 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 11200  & 1400  & 1400  & Yes                  \\
sentiment-2020-rybak-pl           & \cite{rybak-etal-2020-klej}              & pl       & Allegro review            & 2020 & 5        & {Negative, Neutral, Positive, Very\_Negative, Very\_Positive}                                                                                                                                                                                                                  & 8619   & 958   & 1002  & Yes                  \\
sentiment-2020-wilie-in           & \cite{wong-2020-indonlu}                 & in       & Multiple online platforms & 2019 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 9900   & 1100  & 1260  & Yes                  \\
sentiment-2021-abdul-ar           & \cite{arabert-2021-abdulmageed}          & ar       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 49301  & 4443  & 4933  &                      \\
sentiment-2021-diallo-bm          & \cite{diallo-2021-bambara}               & bm       & Multiple online platforms & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 2436   & 305   & 305   & Yes                  \\
sentiment-2021-khondoker-bn       & \cite{islam-etal-2021-sentnob-dataset}   & bn       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 12575  & 1567  & 1586  & Yes                  \\
sentiment-2021-kulkarni-mr        & \cite{kulkarni-2021-l3cubemahasent}      & mr       & Twitter                   & 2020 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 12114  & 1500  & 2250  & Yes                  \\
sentiment-2022-chakravarthi-kn    & \cite{chakravarthi-2022-dravidian}       & kn       & YouTube comment           & 2019 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 3995   & 505   & 502   & Yes                  \\
sentiment-2022-chakravarthi-ml    & \cite{chakravarthi-2022-dravidian}       & ml       & YouTube comment           & 2019 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 8410   & 1044  & 1039  & Yes                  \\
sentiment-2022-chakravarthi-ta    & \cite{chakravarthi-2022-dravidian}       & ta       & YouTube comment           & 2019 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 24063  & 2966  & 3047  & Yes                  \\
sentiment-2022-muhammad-am        & \cite{yimam-etal-2020-exploring}         & am       & Twitter                   & 2020 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 4787   & 598   & 599   & Yes                  \\
sentiment-2022-muhammad-ar        & \cite{mageed:2022:nadi}                  & ar       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 1500   & 500   & 3000  & Yes                  \\
sentiment-2022-muhammad-ha        & \cite{muhammad-2022-naijasenti}          & ha       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 11337  & 1417  & 1418  & Yes                  \\
sentiment-2022-muhammad-ig        & \cite{muhammad-2022-naijasenti}          & ig       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 8153   & 1019  & 1020  & Yes                  \\
sentiment-2022-muhammad-ma        & \cite{muhammad-2022-naijasenti}          & ma       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 4466   & 558   & 559   & Yes                  \\
sentiment-2022-muhammad-pcm       & \cite{muhammad-2022-naijasenti}          & pcm      & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 4096   & 512   & 513   & Yes                  \\
sentiment-2022-muhammad-rw        & \cite{muhammad-2022-naijasenti}          & rw       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 2641   & 330   & 331   & Yes                  \\
sentiment-2022-muhammad-sw        & \cite{muhammad-2022-naijasenti}          & sw       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 1448   & 181   & 181   & Yes                  \\
sentiment-2022-muhammad-ts        & \cite{muhammad-2022-naijasenti}          & ts       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 643    & 80    & 81    & Yes                  \\
sentiment-2022-muhammad-twi       & \cite{muhammad-2022-naijasenti}          & twi      & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 2784   & 348   & 349   & Yes                  \\
sentiment-2022-muhammad-yo        & \cite{muhammad-2022-naijasenti}          & yo       & Twitter                   & 2021 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 6817   & 852   & 853   & Yes                  \\
sentiment-2022-shode-yo           & \cite{shode-2021-africanlp}              & yo       & Multiple online platforms & 2021 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 800    & 200   & 500   & Yes                  \\
sentiment-2022-suzuki-jp          & \cite{suzuki-etal-2022-japanese}         & jp       & SNS post                  & 2021 & 5        & {Negative, Neutral, Positive, Very\_Negative, Very\_Positive}                                                                                                                                                                                                                  & 30000  & 2500  & 2500  & Yes                  \\
sentiment-2022-winata-ace         & \cite{nusax-2020-genta}                  & ace      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-ban         & \cite{nusax-2020-genta}                  & ban      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-bbc         & \cite{nusax-2020-genta}                  & bbc      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-bjn         & \cite{nusax-2020-genta}                  & bjn      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-bug         & \cite{nusax-2020-genta}                  & bug      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-jv          & \cite{nusax-2020-genta}                  & jv       & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-mad         & \cite{nusax-2020-genta}                  & mad      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-min         & \cite{nusax-2020-genta}                  & min      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-nij         & \cite{nusax-2020-genta}                  & nij      & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2022-winata-su          & \cite{nusax-2020-genta}                  & su       & Human translation         & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 500    & 100   & 400   & Yes                  \\
sentiment-2023-marreddy-te        & \cite{mounika-2022-resource}             & te       & Multiple online platforms & 2022 & 3        & {Negative, Neutral, Positive}                                                                                                                                                                                                                                                  & 24599  & 3510  & 7033  & Yes                  \\
sentiment-tw-2012-thelwall-en     & \cite{thelwall2012sentiment}            & en       & Twitter                   & 2012 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 900    & 100   & 1113  & Yes                  \\
sentiment-yt-2012-thelwall-en     & \cite{thelwall2012sentiment}            & en       & YouTube comment           & 2012 & 2        & {Negative, Positive}                                                                                                                                                                                                                                                           & 900    & 100   & 1142  & Yes                  \\
sentiment5-2013-socher-en         & \cite{socher-2013-recursive}             & en       & Moview review             & 2013 & 5        & {Negative, Neutral, Positive, Very\_Negative, Very\_Positive}                                                                                                                                                                                                                  & 8544   & 1101  & 2210  & Yes                  \\
sexism-2020-chiril-fr             & \cite{chiril2020annotated}               & fr       & Twitter                   & 2018 & 2        & {Not, Sexism}                                                                                                                                                                                                                                                                  & 7670   & 959   & 959   & Yes                  \\
stance-2016-mohammad-en           & \cite{mohammad-2016-semeval}             & en       & Twitter                   & 2016 & 3        & {Against, Favor, Not}                                                                                                                                                                                                                                                          & 2622   & 292   & 1249  & Yes                  \\
subjective-2013-kosac-ko          & \cite{jang-2013-kosac}                   & ko       & News articles             & 2013 & 7        & {Agreement, Argument, Emotion, Intention, Judgment, Others, Speculation}                                                                                                                                                                                                       & 4284   & 535   & 536   & No                   \\
subjective-2016-barbieri-es       & \cite{barbieri2016overview}              & es       & Twitter                   & 2014 & 2        & {Objective, Subjective}                                                                                                                                                                                                                                                        & 6669   & 741   & 1998  & Yes                  \\ \bottomrule
\end{tabular}
\caption{Summary of datasets in our benchmark.}\label{tab:data_sum}
\end{table*}

==> table_fig/dev_res.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{@{}llcccccc|c@{}}
\toprule
                                           & \multicolumn{1}{c}{\textbf{Tasks}} & \multicolumn{1}{c}{\textbf{mBERT}} & \multicolumn{1}{c}{\textbf{XLM-R\textsubscript{B}}} & \multicolumn{1}{c}{\textbf{XLM-T}} & \multicolumn{1}{c}{\textbf{TwHIN-BERT}} & \multicolumn{1}{c}{\textbf{Bernice}} & \multicolumn{1}{c|}{\textbf{SLP}}   & \multicolumn{1}{c}{\textbf{XLM-R\textsubscript{L}}} \\ \midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Anti-social}}}       & Aggregate                         & 73.39 & 73.92                                   & 75.55 & 73.77      & \textbf{76.79}   & 75.61 &  \underline{76.94}                                   \\
                                           & Dangerous                         & 69.76 & 69.53                                   & \textbf{75.06} & 71.35      & 74.92   & 74.31 & 70.43                                   \\
                                           & Hate Speech                              & 78.15 & 79.82                                   & 80.49 & 81.28      & \textbf{81.43}   & 80.04 &  81.15                                   \\
                                           & Offensive                            & 78.96 & 80.21                                   & 81.50 & 81.57      & \textbf{82.15}   & 81.38 & 81.02                                   \\
                                           & H/O-Group                          & \textbf{51.57} & 41.24                                   & 49.67 & 45.07      & 48.30   & 44.63 &  51.08                                   \\
                                           & H/O-Target                         & 54.02 & 59.23                                   & 58.16 & 59.95      & \textbf{60.83}   & 59.50 & \underline{62.04}                                   \\ \cdashline{2-9}
                                           & \textbf{AS}                        & 70.14 & 71.42                                   & 72.65 & 72.86      & \textbf{73.71}   & 72.29 & \underline{73.75}                                   \\\hline
\multicolumn{2}{l}{\textbf{Emotion}}                                            & 56.17 & 61.68                                   & 63.05 & 61.45      & 62.70   & \textbf{63.95} &  \underline{66.12}                                   \\\hline
\multicolumn{2}{l}{\textbf{Humor}}                                              & 85.15 & 85.83                                   & 86.55 & 86.18      & \textbf{86.72}   & 85.99 &  \underline{87.59}                                   \\\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{I\&S}}} & Irony                              & 70.18 & 70.80                                   & 72.42 & 71.60      & \textbf{72.75}   & 71.96 & 71.77                                   \\
                                           & Sarcasm                            & 74.65 & 75.64                                   & 77.44 & 76.26      & \textbf{77.82}   & 77.15 &  \underline{78.52}                                   \\
                                           & Irony-Target                         & 53.51 & 52.18                                   & \textbf{59.08} & 53.67      & 58.55   & 56.91 & 56.71                                   \\ \cdashline{2-9}
                                           & \textbf{I\&S}                      & 71.66 & 72.37                                   & 74.36 & 73.11      & \textbf{74.67}   & 73.90 & 74.53                                   \\\hline
\multicolumn{2}{l}{\textbf{Sentiment}}                                          & 68.84 & 70.79                                   & 72.16 & 71.25      & 72.29   & \textbf{73.05} &  72.95                                   \\\hline
\multicolumn{2}{l}{\textbf{Subjectivity}}                                       & 74.80 & 76.28                                   & \textbf{76.53} & 73.94      & 75.21   & 76.21 &  \underline{78.19}                                   \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{l}{\textbf{SPARROW}}                                                 & 68.91 & 70.84                                   & 72.20 & 71.42      & 72.49   & \textbf{72.56} & \underline{73.23}                                   \\ \bottomrule
\end{tabular}
\caption{Dev results of SPARROW benchmark. We report the average of dataset-specific metrics in a task and a category, respectively.}\label{tab:dev_res}
\end{table*}

==> table_fig/emotion_prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{ll}
\toprule
\textbf{Dataset}	 & \textbf{Prompt}	\\ \midrule
Emot-eng\textsubscript{Wal}, Emot-zho\textsubscript{Lee}, Emot-fin\textsubscript{Kaj}, Emot-fre\textsubscript{Kaj}, Emot-ita\textsubscript{Kaj}, Emot-msa\textsubscript{Hus}, Emot-ara\textsubscript{Abd} 	 & 	\multirow{4}{*}{\makecell[l]{\{Content\} \\ Question: Is the emotion of this sentence \{labels\}? \\ Answer: }} \\ 
Emot-eng\textsubscript{Moh}, Emot-ara\textsubscript{Moh}, Emot-spa\textsubscript{Moh}, Emot-ind\textsubscript{Sap}, Emot-tur\textsubscript{Guv}, Emot-spa\textsubscript{Moh}, Emot-ind\textsubscript{Wil} 	 & 	\\ 
Emot-vie\textsubscript{Ho}, Emot-eng\textsubscript{Pla}, Emot-spa\textsubscript{Pla}, Emot-fin\textsubscript{Ohm}, Emot-eng\textsubscript{Dem}, Emot-ita\textsubscript{Bia}, Emot-ron\textsubscript{Cio} 	 & 	\\ 
Emot-hin\textsubscript{Deb}, Emot-por\textsubscript{Cor}, Emot-fas\textsubscript{Sab}, Emot-rus\textsubscript{Sbo}, Emot-ben\textsubscript{Iqb}, Emot-fre\textsubscript{Bia}, Emot-deu\textsubscript{Bia} 	 & 	\\
\bottomrule 
\end{tabular}
\caption{Emotion} \label{tab:emotion_prompt}
\end{table*}

==> table_fig/humor_prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{p{0.1\linewidth}l}
 \toprule
\textbf{Dataset}	 & \textbf{Prompt}\\ \midrule
Humo-hin\textsubscript{Agg} & \multirow{4}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\ 
Humo-rus\textsubscript{Bli} & 	\\ 
Humo-spa\textsubscript{Chi} & 	\\ 
Humo-eng\textsubscript{Mea} & 	\\ 
\bottomrule 
\end{tabular}
\caption{Humor}\label{tab:humor_prompt}
\end{table*}

==> table_fig/irony_prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{p{0.1\linewidth}l}
 \toprule
\textbf{Dataset}	 & \textbf{Prompt}\\ \midrule
Iron-ita\textsubscript{Bas} 	 & \multirow{20}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\ 
Iron-spa\textsubscript{Bar} 	 & \\ 
Iron-eng\textsubscript{Hee} 	 & \\ 
Iron-ita\textsubscript{Cig} 	 & \\ 
Iron-hin\textsubscript{Vij} 	 & \\ 
Iron-ara\textsubscript{Gha} 	 & \\ 
Iron-spa\textsubscript{Ort} 	 & \\ 
Iron-fas\textsubscript{Gol}\textsuperscript{$\star$} 	 & \\ 
Iron-zho\textsubscript{Xia}\textsuperscript{$\star$} 	 & \\  
% \midrule
Sarc-eng\textsubscript{Wal} 	 & \\ 
Sarc-eng\textsubscript{Ril} 	 & \\ 
Sarc-ces\textsubscript{Pta} 	 & \\ 
Sarc-eng\textsubscript{Pta} 	 & \\ 
Sarc-eng\textsubscript{Bam} 	 & \\ 
Sarc-eng\textsubscript{Raj} 	 & \\ 
Sarc-eng\textsubscript{Ora} 	 & \\ 
Sarc-zho\textsubscript{Gon}\textsuperscript{$\star$} 	 & \\ 
Sarc-ara\textsubscript{Abu} 	 & \\ 
Sarc-ara\textsubscript{Far} 	 & \\ 
Iron-T-eng\textsubscript{Hee} 	 & \makecell[l]{\{Content\} \\ Question: Is the type of this text \{labels\}? \\ Answer: } \\
\bottomrule 
\end{tabular}
\caption{Irony}\label{tab:irony_prompt}
\end{table*}


==> table_fig/prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{lcll}
 \toprule
 & \multicolumn{2}{l}{\textbf{Dataset}}	 & \textbf{Prompt} \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{27}{*}{\rotatebox[origin=c]{90}{\textbf{Anti-social}}} & \multicolumn{2}{l}{Dang-ara\textsubscript{Als}} 	 & \makecell[l]{\{Content\} \\ Question: Is the language of this sentence \{labels\}? \\ Answer: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Aggr-hin\textsubscript{Kum}, Hate-eng\textsubscript{Dav}, Hate-eng\textsubscript{Was}, Hate-ara\textsubscript{Ala}, Hate-ita\textsubscript{Bos}\textsuperscript{$\star$}, Hate-fil\textsubscript{Cab}} 	 & \multirow{4}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\
& \multicolumn{2}{l}{Hate-ara\textsubscript{Mul}, Hate-eng\textsubscript{Bas}, Hate-spa\textsubscript{Bas}, Hate-por\textsubscript{For}, Hate-pol\textsubscript{Pta}, Hate-kor\textsubscript{Moo}} 	 & \\
& \multicolumn{2}{l}{Hate-ara\textsubscript{Mub}, Hate-zho\textsubscript{Den}, Hate-kor\textsubscript{Jeo}, Hate-tel\textsubscript{Mar}, Sexi-fre\textsubscript{Chi}, Offe-eng\textsubscript{Zam}} 	 & \\ 
& \multicolumn{2}{l}{Offe-ara\textsubscript{Zam}, Offe-dan\textsubscript{Zam}, Offe-ell\textsubscript{Zam}, Offe-tur\textsubscript{Zam}, Offe-ara\textsubscript{Mub}, Offe-slv\textsubscript{Nov}} 	 & \\ \noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Offe-T-kan\textsubscript{Cha}, Offe-G-eng\textsubscript{Zam}, Hate-T-kor\textsubscript{Jeo}} 	 & \makecell[l]{\{Content\} \\ Question: Does this offensive text target \{labels\}? \\ Answers: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Hate-G-ara\textsubscript{Ous}, Hate-G-fre\textsubscript{Ous}} 	 & \makecell[l]{\{Content\} \\ Question: Does this hate speech target \{labels\}? \\ Answer: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Offe-T-eng\textsubscript{Zam}} 	 & \makecell[l]{\{Content\} \\ Question: Is this offensive text \{labels\} insult? \\ Answer: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Hate-T-ara\textsubscript{Ous}, Hate-T-fre\textsubscript{Ous}} 	 & \makecell[l]{\{Content\} \\ Question: Does this hate speech text insult against people based on \\ their attribute of \{labels\}? \\ Answer: }
\\ \noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Hate-T-ben\textsubscript{Kar}} 	 & \makecell[l]{\{Content\} \\ Question: Does this text express \{labels\}? \\ Answer: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Offe-T-mal\textsubscript{Cha}, Offe-T-tam\textsubscript{Cha}} 	 & \makecell[l]{\{Content\} \\ Question: Is this sentence hate speech or not? If yes, does this sentence \\ target individual, group or not? \\ Answer: } \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Emotion}}} & \multicolumn{2}{l}{Emot-eng\textsubscript{Wal}, Emot-zho\textsubscript{Lee}, Emot-fin\textsubscript{Kaj}, Emot-fre\textsubscript{Kaj}, Emot-ita\textsubscript{Kaj}, Emot-msa\textsubscript{Hus}, Emot-ara\textsubscript{Abd}} 	 & 	\multirow{4}{*}{\makecell[l]{\{Content\} \\ Question: Is the emotion of this sentence \{labels\}? \\ Answer: }} \\ 
& \multicolumn{2}{l}{Emot-eng\textsubscript{Moh}, Emot-ara\textsubscript{Moh}, Emot-spa\textsubscript{Moh}, Emot-ind\textsubscript{Sap}, Emot-tur\textsubscript{Guv}, Emot-spa\textsubscript{Moh}, Emot-ind\textsubscript{Wil}} 	 & 	\\ 
& \multicolumn{2}{l}{Emot-vie\textsubscript{Ho}, Emot-eng\textsubscript{Pla}, Emot-spa\textsubscript{Pla}, Emot-fin\textsubscript{Ohm}, Emot-eng\textsubscript{Dem}, Emot-ita\textsubscript{Bia}, Emot-ron\textsubscript{Cio}} 	 & 	\\ 
& \multicolumn{2}{l}{Emot-hin\textsubscript{Deb}, Emot-por\textsubscript{Cor}, Emot-fas\textsubscript{Sab}, Emot-rus\textsubscript{Sbo}, Emot-ben\textsubscript{Iqb}, Emot-fre\textsubscript{Bia}, Emot-deu\textsubscript{Bia}} 	 & 	\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\rotatebox[origin=c]{90}{\textbf{Humor}} & \multicolumn{2}{l}{Humo-hin\textsubscript{Agg}, Humo-rus\textsubscript{Bli}, Humo-spa\textsubscript{Chi}, Humo-eng\textsubscript{Mea}} & \makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: } \\
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Irony}}} & \multicolumn{2}{l}{Iron-ita\textsubscript{Bas}, Iron-spa\textsubscript{Bar}, Iron-eng\textsubscript{Hee}, Iron-ita\textsubscript{Cig}, Iron-hin\textsubscript{Vij}, Iron-ara\textsubscript{Gha}, Iron-spa\textsubscript{Ort}} & \multirow{3}{*}{\makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }} \\
& \multicolumn{2}{l}{Iron-fas\textsubscript{Gol}\textsuperscript{$\star$}, Iron-zho\textsubscript{Xia}\textsuperscript{$\star$}, Sarc-eng\textsubscript{Wal}, Sarc-eng\textsubscript{Ril}, Sarc-ces\textsubscript{Pta}, Sarc-eng\textsubscript{Pta}, Sarc-eng\textsubscript{Bam}} \\
& \multicolumn{2}{l}{Sarc-eng\textsubscript{Raj}, Sarc-eng\textsubscript{Ora}, Sarc-zho\textsubscript{Gon}\textsuperscript{$\star$}, Sarc-ara\textsubscript{Abu}, Sarc-ara\textsubscript{Far}} \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Iron-T-eng\textsubscript{Hee}} 	 & \makecell[l]{\{Content\} \\ Question: Is the type of this text \{labels\}? \\ Answer: } \\
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{13}{*}{\rotatebox[origin=c]{90}{\textbf{Sentiment}}} & \multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Sentiment Analysis}}} & Sent-eng\textsubscript{Pan}, Sent-zho\textsubscript{Tan}, Sent-kor\textsubscript{Jan}, Sent-eng\textsubscript{Soc}, Sent-ita\textsubscript{Bas}, Sent-ben\textsubscript{Pat}, Sent-hin\textsubscript{Pat} & \multirow{10}{*}{\makecell[l]{\{Content\} \\ Question: Is the sentiment of this sentence \{labels\}? \\ Answer: }}	\\
& & Sent-ita\textsubscript{Bas}, Sent-mlt\textsubscript{Din}, Sent-bul\textsubscript{Moz}, Sent-bos\textsubscript{Moz}, Sent-deu\textsubscript{Moz}, Sent-eng\textsubscript{Moz}, Sent-spa\textsubscript{Moz} & \\
& & Sent-hrv\textsubscript{Moz}, Sent-hun\textsubscript{Moz}, Sent-pol\textsubscript{Moz}, Sent-por\textsubscript{Moz}, Sent-rus\textsubscript{Moz}, Sent-slk\textsubscript{Moz}, Sent-slv\textsubscript{Moz} & \\
& & Sent-sqi\textsubscript{Moz}, Sent-srp\textsubscript{Moz}, Sent-swe\textsubscript{Moz}, Sent-deu\textsubscript{Rei}, Sent-spa\textsubscript{Rei}, Sent-ita\textsubscript{Rei}, Sent-eng\textsubscript{Ros} & \\
& & Sent-heb\textsubscript{Amr}, Sent-por\textsubscript{Bru}, Sent-fin\textsubscript{Kaj}, Sent-fre\textsubscript{Kaj}, Sent-ita\textsubscript{Kaj}, Sent-pol\textsubscript{Koc}, Sent-tha\textsubscript{Sur} & \\
& & Sent-zho\textsubscript{Wan}, Sent-fas\textsubscript{Ash}, Sent-ron\textsubscript{Dum}, Sent-pcm\textsubscript{Oye}, Sent-pol\textsubscript{Ryb}, Sent-ind\textsubscript{Wil}, Sent-ara\textsubscript{Abd} & \\
& & Sent-bam\textsubscript{Dia}, Sent-ben\textsubscript{Isl}, Sent-mar\textsubscript{Kul}, Sent-kan\textsubscript{Cha}, Sent-mal\textsubscript{Cha}, Sent-tam\textsubscript{Cha}, Sent-ara\textsubscript{Muh} & \\
& & Sent-amh\textsubscript{Muh}, Sent-ary\textsubscript{Muh}, Sent-arq\textsubscript{Muh}, Sent-hau\textsubscript{Muh}, Sent-ibo\textsubscript{Muh}, Sent-pcm\textsubscript{Muh}, Sent-kin\textsubscript{Muh} & \\
& & Sent-swh\textsubscript{Muh}, Sent-tso\textsubscript{Muh}, Sent-twi\textsubscript{Muh}, Sent-yor\textsubscript{Muh}, Sent-yor\textsubscript{Sho}, Sent-jpn\textsubscript{Suz}, Sent-ace\textsubscript{Win} & \\
& & Sent-ban\textsubscript{Win}, Sent-bbc\textsubscript{Win}, Sent-bjn\textsubscript{Win}, Sent-bug\textsubscript{Win}, Sent-jav\textsubscript{Win}, Sent-mad\textsubscript{Win}, Sent-min\textsubscript{Win} & \\
& & Sent-nij\textsubscript{Win}, Sent-sun\textsubscript{Win}, Sent-tel\textsubscript{Mar}, Sent-T-eng\textsubscript{The}, Sent-Y-eng\textsubscript{The}, Sent-5-eng\textsubscript{Soc} & \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Sent-nor\textsubscript{Vel}} 	 & 	\makecell[l]{\{Content\} \\ Question: Is this text rated as \{labels\}? Higher is better. \\ Answer: } \\
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Subjective}}} & \multicolumn{2}{l}{Subj-kor\textsubscript{Jan}} & \makecell[l]{\{Content\} \\ Question: Does this sentence express \{labele\}? \\ Answer: } \\
\noalign{\smallskip}\cline{2-4}\noalign{\smallskip}
& \multicolumn{2}{l}{Subj-eng\textsubscript{Pan}, Subj-ita\textsubscript{Bas}, Subj-ita\textsubscript{Bas}, Subj-spa\textsubscript{Bar}, Subj-ces\textsubscript{Pri}} & \makecell[l]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: } \\
\bottomrule 
\end{tabular}
\caption{Prompts.}\label{tab:prompt}
\end{table*}




==> table_fig/sentiment_prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{p{0.1\linewidth}l}
 \toprule
\textbf{Dataset}	 & \textbf{Prompt}	 \\ \midrule
Sent-eng\textsubscript{Pan} 	 &  \multirow{76}{*}{\makecell[l]{\{Content\} \\ Question: Is the sentiment of this sentence \{labels\}? \\ Answer: }}	\\ 
Sent-zho\textsubscript{Tan} 	 & 	\\ 
Sent-kor\textsubscript{Jan} 	 & 	\\ 
Sent-eng\textsubscript{Soc} 	 & 	\\ 
Sent-ita\textsubscript{Bas} 	 & 	\\ 
Sent-ben\textsubscript{Pat} 	 & 	\\ 
Sent-hin\textsubscript{Pat} 	 & 	\\ 
Sent-ita\textsubscript{Bas} 	 & 	\\ 
Sent-mlt\textsubscript{Din} 	 & 	\\ 
Sent-bul\textsubscript{Moz} 	 & 	\\ 
Sent-bos\textsubscript{Moz} 	 & 	\\ 
Sent-deu\textsubscript{Moz} 	 & 	\\ 
Sent-eng\textsubscript{Moz} 	 & 	\\ 
Sent-spa\textsubscript{Moz} 	 & 	\\ 
Sent-hrv\textsubscript{Moz} 	 & 	\\ 
Sent-hun\textsubscript{Moz} 	 & 	\\ 
Sent-pol\textsubscript{Moz} 	 & 	\\ 
Sent-por\textsubscript{Moz} 	 & 	\\ 
Sent-rus\textsubscript{Moz} 	 & 	\\ 
Sent-slk\textsubscript{Moz} 	 & 	\\ 
Sent-slv\textsubscript{Moz} 	 & 	\\ 
Sent-sqi\textsubscript{Moz} 	 & 	\\ 
Sent-srp\textsubscript{Moz} 	 & 	\\ 
Sent-swe\textsubscript{Moz} 	 & 	\\ 
Sent-deu\textsubscript{Rei} 	 & 	\\ 
Sent-spa\textsubscript{Rei} 	 & 	\\ 
Sent-ita\textsubscript{Rei} 	 & 	\\ 
Sent-eng\textsubscript{Ros} 	 & 	\\ 
Sent-heb\textsubscript{Amr} 	 & 	\\ 
Sent-por\textsubscript{Bru} 	 & 	\\ 
Sent-fin\textsubscript{Kaj} 	 & 	\\ 
Sent-fre\textsubscript{Kaj} 	 & 	\\ 
Sent-ita\textsubscript{Kaj} 	 & 	\\ 
Sent-pol\textsubscript{Koc} 	 & 	\\ 
Sent-tha\textsubscript{Sur} 	 & 	\\ 
Sent-zho\textsubscript{Wan} 	 & 	\\ 
Sent-fas\textsubscript{Ash} 	 & 	\\ 
Sent-ron\textsubscript{Dum} 	 & 	\\ 
Sent-pcm\textsubscript{Oye} 	 & 	\\ 
Sent-pol\textsubscript{Ryb} 	 & 	\\ 
Sent-ind\textsubscript{Wil} 	 & 	\\ 
Sent-ara\textsubscript{Abd} 	 & 	\\ 
Sent-bam\textsubscript{Dia} 	 & 	\\ 
Sent-ben\textsubscript{Isl} 	 & 	\\ 
Sent-mar\textsubscript{Kul} 	 & 	\\ 
Sent-kan\textsubscript{Cha} 	 & 	\\ 
Sent-mal\textsubscript{Cha} 	 & 	\\ 
Sent-tam\textsubscript{Cha} 	 & 	\\ 
Sent-ara\textsubscript{Muh} 	 & 	\\ 
Sent-amh\textsubscript{Muh} 	 & 	\\ 
Sent-ary\textsubscript{Muh} 	 & 	\\ 
Sent-arq\textsubscript{Muh} 	 & 	\\ 
Sent-hau\textsubscript{Muh} 	 & 	\\ 
Sent-ibo\textsubscript{Muh} 	 & 	\\ 
Sent-pcm\textsubscript{Muh} 	 & 	\\ 
Sent-kin\textsubscript{Muh} 	 & 	\\ 
Sent-swh\textsubscript{Muh} 	 & 	\\ 
Sent-tso\textsubscript{Muh} 	 & 	\\ 
Sent-twi\textsubscript{Muh} 	 & 	\\ 
Sent-yor\textsubscript{Muh} 	 & 	\\ 
Sent-yor\textsubscript{Sho} 	 & 	\\ 
Sent-jpn\textsubscript{Suz} 	 & 	\\ 
Sent-ace\textsubscript{Win} 	 & 	\\ 
Sent-ban\textsubscript{Win} 	 & 	\\ 
Sent-bbc\textsubscript{Win} 	 & 	\\ 
Sent-bjn\textsubscript{Win} 	 & 	\\ 
Sent-bug\textsubscript{Win} 	 & 	\\ 
Sent-jav\textsubscript{Win} 	 & 	\\ 
Sent-mad\textsubscript{Win} 	 & 	\\ 
Sent-min\textsubscript{Win} 	 & 	\\ 
Sent-nij\textsubscript{Win} 	 & 	\\ 
Sent-sun\textsubscript{Win} 	 & 	\\ 
Sent-tel\textsubscript{Mar} 	 & 	\\ 
Sent-T-eng\textsubscript{The} 	 & 	\\ 
Sent-Y-eng\textsubscript{The} 	 & 	\\ 
Sent-5-eng\textsubscript{Soc} 	 & 	\\ \midrule
Sent-nor\textsubscript{Vel} 	 & 	\makecell[l]{\{Content\} \\ Question: Is this text rated as \{labels\}? Higher is better. \\ Answer: } \\
\bottomrule 
\end{tabular}
\caption{Full test results on sentiment analysis task. \textbf{SoTA:} Previous SoTA performance on each respective dataset. \textbf{Underscore} indicates that our models are trained on different data splits to the SoTA model. } \label{tab:sentiment_res}
\end{table*}


==> table_fig/subject_prompt.tex <==
\begin{table*}[h]
\centering 
\tiny
\begin{tabular}{@{}llccccccc|cl@{}}
 \toprule
\textbf{Dataset}	 & \textbf{Prompt}	 \\ \midrule
Subj-kor\textsubscript{Jan} 	 & 	\makecell[l]{\{Content\} \\ Question: Does this sentence express \{labele\}? \\ Answer: }\\ \midrule 
Subj-eng\textsubscript{Pan} 	 &  \multirow{5}{*}{\makecell[*]{\{Content\} \\ Question: Is this sentence \{labels\}? \\ Answer: }}	\\ 
Subj-ita\textsubscript{Bas} 	 & 	\\ 
Subj-ita\textsubscript{Bas} 	 & 	\\ 
Subj-spa\textsubscript{Bar} 	 & 	\\ 
Subj-ces\textsubscript{Pri} 	 & 	\\
\bottomrule 
\end{tabular}
\caption{Subjective} \label{tab:subjectivity_prompt}
\end{table*}



==> zero-shot_eval.tex <==
\section{Zero-shot Evaluation Process}
We conducted a zero-shot evaluation on various types of models, including sequence-to-sequence encoder-decoder models (mt5-base, mt5-xl, mt0-base, mt0-xl), auto-regressive models (bloom-base, bloom-7b1, bloomz-base, bloomz-7b1, bloomz-7b1-p3, LLaMa, Vicuna, Bactrian-X, and Alpaca), and encoder-only models (mbert, xlm-r, xlmr-tw, and bernice).

To assess these models, we utilized datasets divided into six distinct categories: Anti-social, Emotion, Humor, Irony, Sentiment Analysis, and Subjective. Within each category, we defined specific subcategories. During the evaluation process, we employed different prompts tailored to each subcategory. These prompts resembled question-and-answer tasks, where we provided the content and question, and asked the model to generate an answer based on the provided labels. The labels served as candidate answers, and we calculated the log-likelihood for each candidate. The prediction with the highest log-likelihood was selected as the model's output, which was then compared to the gold label to evaluate the performance. Various evaluation metrics were used for different tasks, but the most common metric in our experiment was the Micro-F1 score.
